Exploiting Spatial-temporal Data for Sleep Stage Classification via Hypergraph Learning

Sleep stage classification is crucial for detecting patients' health conditions. Existing models, which mainly use Convolutional Neural Networks (CNN) for modelling Euclidean data and Graph Convolution Networks (GNN) for modelling non-Euclidean data, are unable to consider the heterogeneity and interactivity of multimodal data as well as the spatial-temporal correlation simultaneously, which hinders a further improvement of classification performance. In this paper, we propose a dynamic learning framework STHL, which introduces hypergraph to encode spatial-temporal data for sleep stage classification. Hypergraphs can construct multi-modal/multi-type data instead of using simple pairwise between two subjects. STHL creates spatial and temporal hyperedges separately to build node correlations, then it conducts type-specific hypergraph learning process to encode the attributes into the embedding space. Extensive experiments show that our proposed STHL outperforms the state-of-the-art models in sleep stage classification tasks.

==> model.tex <==
import math
import matplotlib.pyplot as plt
import dhg
import torch
import torch.nn as nn
import torch.nn.functional as F


class Predictor(nn.Module):
    def __init__(self,in_dim,n_cats):
        super(Predictor, self).__init__()
        self.predict = nn.Linear(in_dim,n_cats)
        torch.nn.init.xavier_uniform_(self.predict.weight)
        self.sigma =  nn.Sigmoid()
        self.softmax = nn.Softmax()

    def forward(self,node_emb):
        n_cat = self.predict(node_emb)
        # n_cat = self.sigma(n_cat)
        # n_cat = self.softmax(n_cat)
        return n_cat

class Readout(nn.Module):
    def __init__(self,in_dim,method = "mean"):
        super(Readout, self).__init__()
        self.method = method
        self.linear = nn.Linear(2*in_dim,in_dim)
        nn.init.xavier_normal_(self.linear.weight)


    def forward(self,node_fea,raw):
        if self.method == "mean":
            return torch.mean(self.linear(torch.hstack([node_fea,raw])), dim=0)

class SpatialHyperedge(nn.Module):
    def __init__(self,in_dim,l2_lamda = 0.001,recons_lamda = 0.2,num_node = 10,lb_th = 0):
        super(SpatialHyperedge, self).__init__()
        self.l2_lamda = l2_lamda
        self.recons_lamda = recons_lamda
        # projection matrix
        self.num_node = num_node
        self.r_proj = nn.Parameter(torch.nn.init.xavier_uniform_(torch.rand(in_dim,in_dim)))
        # reconstruction linear combination
        self.incidence_m = nn.Parameter(torch.nn.init.xavier_uniform_(torch.rand(num_node,num_node-1)))
        self.lb_th = lb_th

    def forward(self,X):
        self.incidence_all = torch.zeros(self.num_node, self.num_node)
        self_node = torch.eye(self.num_node)
        self.recon_loss = 0
        X = X.detach()
        for node_idx in range(self.num_node):
            master_node_fea = X[node_idx]
            master_node_proj_fea = torch.matmul(master_node_fea, self.r_proj).reshape(1, -1)
            slave_node_idx = [i for i in range(self.num_node) if i != node_idx]
            node_linear_comb = self.incidence_m[node_idx].unsqueeze(0)
            node_linear_comb = torch.clamp(node_linear_comb, min=self.lb_th)

            node_linear_comb_mask = node_linear_comb > self.lb_th
            node_linear_comb = node_linear_comb.masked_fill(~node_linear_comb_mask, value=torch.tensor(0))
            neigh_recon_fea = torch.matmul(node_linear_comb, X[slave_node_idx])
            self.incidence_all[node_idx][slave_node_idx] = node_linear_comb
            linear_comb_l1 = torch.linalg.norm(node_linear_comb, 1)
            linear_comb_l2 = torch.linalg.norm(node_linear_comb, 2)

            recon_error = torch.linalg.norm(master_node_proj_fea - neigh_recon_fea, 2)
                # recon_error = torch.cdist(master_node_proj_fea,neigh_recon_fea,2)
                # linear_comb_l1 = torch.linalg.norm(self.incidence_m[neigh_recon_idx],1)
                # linear_comb_l2 = torch.linalg.norm(self.incidence_m[neigh_recon_idx],2)
            node_recons_loss = recon_error * self.recons_lamda + linear_comb_l1 + self.l2_lamda * linear_comb_l2
                # node_recons_loss = recon_error.squeeze()
            self.recon_loss += node_recons_loss
        self.incidence_all = self.incidence_all + self_node
        return self.recon_loss, self.incidence_all

class TemporalHyperedge(nn.Module):
    def __init__(self,in_dim,l2_lamda = 0.001,recons_lamda = 0.2,num_node = 10,lb_th = 0):
        super(TemporalHyperedge, self).__init__()
        self.l2_lamda = l2_lamda
        self.recons_lamda = recons_lamda
        # projection matrix
        self.num_node = num_node
        self.r_proj = nn.Parameter(torch.nn.init.xavier_uniform_(torch.rand(in_dim,in_dim)))
        # reconstruction linear combination
        self.incidence_m = nn.Parameter(torch.nn.init.xavier_uniform_(torch.rand(num_node,num_node)))
        self.lb_th = lb_th

    def forward(self,cur,pre):
        # self.incidence_all = torch.zeros(self.num_node, self.num_node)
        self_node = torch.eye(self.num_node)
        self.recon_loss = 0
        cur = cur.detach()
        pre = pre.detach()
        for node_idx in range(self.num_node):
            master_node_fea = cur[node_idx]
            master_node_proj_fea = torch.matmul(master_node_fea, self.r_proj).reshape(1, -1)
            slave_node_idx = [i for i in range(self.num_node)]
            node_linear_comb = self.incidence_m[node_idx].unsqueeze(0)
            node_linear_comb = torch.clamp(node_linear_comb, min=self.lb_th)

            node_linear_comb_mask = node_linear_comb > self.lb_th
            node_linear_comb = node_linear_comb.masked_fill(~node_linear_comb_mask, value=torch.tensor(0))
            neigh_recon_fea = torch.matmul(node_linear_comb,pre)
            # self.incidence_all[node_idx][slave_node_idx] = node_linear_comb
            linear_comb_l1 = torch.linalg.norm(node_linear_comb, 1)
            linear_comb_l2 = torch.linalg.norm(node_linear_comb, 2)

            recon_error = torch.linalg.norm(master_node_proj_fea - neigh_recon_fea, 2)
                # recon_error = torch.cdist(master_node_proj_fea,neigh_recon_fea,2)
                # linear_comb_l1 = torch.linalg.norm(self.incidence_m[neigh_recon_idx],1)
                # linear_comb_l2 = torch.linalg.norm(self.incidence_m[neigh_recon_idx],2)
            node_recons_loss = recon_error * self.recons_lamda + linear_comb_l1 + self.l2_lamda * linear_comb_l2
                # node_recons_loss = recon_error.squeeze()
            self.recon_loss += node_recons_loss
        # self.incidence_all = self.incidence_all + self_node
        return self.recon_loss, self.incidence_m

class SpatialHyperedgeMP(nn.Module):
    def __init__(self):
        super(SpatialHyperedgeMP, self).__init__()

    def forward(self,cur,incidence_m):
        edge_fea = torch.mm(incidence_m, cur)
        edge_degree = torch.sum(incidence_m, dim=1).reshape(-1, 1)
        edge_fea_normed = torch.div(edge_fea,edge_degree)
        return edge_fea_normed

class TemporalHyperedgeMP(nn.Module):
    def __init__(self):
        super(TemporalHyperedgeMP, self).__init__()

    def forward(self,cur,pre,incidence_m):
        edge_fea = torch.mm(incidence_m, pre) + cur
        self_degree = torch.ones(incidence_m.shape[0],1)
        edge_degree = torch.sum(incidence_m, dim=1).reshape(-1, 1) + self_degree
        edge_fea_normed = torch.div(edge_fea,edge_degree)
        return edge_fea_normed

class HHNodeMP(nn.Module):
    def __init__(self,in_dim = 256,num_node = 10,drop_rate = 0.3):
        super(HHNodeMP, self).__init__()
        self.node_proj = nn.Parameter(torch.nn.init.xavier_uniform_(torch.rand(in_dim,in_dim)))
        self.spatial_edge_proj = nn.Parameter(torch.nn.init.xavier_uniform_(torch.rand(in_dim,in_dim)))
        self.temporal_edge_proj = nn.Parameter(torch.nn.init.xavier_uniform_(torch.rand(in_dim,in_dim)))
        self.num_node = num_node
        self.act_1 = nn.Softmax(dim = 0)
        self.in_dim = in_dim
        self.drop = nn.Dropout(drop_rate)
        self.act = nn.ReLU(inplace=True)
        self.theta = nn.Linear(in_dim, in_dim, bias=True)
        torch.nn.init.xavier_uniform_(self.theta.weight)


    def forward(self,cur,spatial_hyperedge_emb,temporal_hyperedge_emb):
        rlt = []
        for node_idx in range(self.num_node):
            node_fea = cur[node_idx]
            node_fea = torch.matmul(node_fea, self.node_proj)
            spatial_hyperedge_fea = spatial_hyperedge_emb[node_idx]
            temporal_hyperedge_fea = temporal_hyperedge_emb[node_idx]
            spatial_hyperedge_fea = torch.matmul(spatial_hyperedge_fea, self.spatial_edge_proj)
            temporal_hyperedge_fea = torch.matmul(temporal_hyperedge_fea, self.temporal_edge_proj)
            hyperedge = torch.vstack([spatial_hyperedge_fea,temporal_hyperedge_fea])
            atten = self.act_1(torch.matmul(hyperedge,node_fea.T)/math.sqrt(self.in_dim)).reshape(-1,1)
            rlt.append(torch.sum(torch.mul(atten,hyperedge),0).reshape(1,-1))
        return self.drop(self.act(self.theta(torch.vstack(rlt))))



class TimeBlock(nn.Module):
    def __init__(self,in_dim = 256,num_node = 10):
        super(TimeBlock, self).__init__()
        self.spatial_hyperedge = SpatialHyperedge(in_dim)
        self.temporal_hyperedge = TemporalHyperedge(in_dim)
        self.spatial_hyperedge_MP = SpatialHyperedgeMP()
        self.temporal_hyperedge_MP = TemporalHyperedgeMP()
        self.node_mp = HHNodeMP()

    def forward(self,cur,pre):
        """
        :param cur: N * d
        :param pred: N * d
        :return: N * d
        """
        spatial_hyperedge_loss,spatial_hyperedge_incidence = self.spatial_hyperedge(cur)
        temporal_hyperedge_loss, temporal_hyperedge_incidence = self.temporal_hyperedge(cur,pre)
        spatial_hyperedge_emb = self.spatial_hyperedge_MP(cur,spatial_hyperedge_incidence)
        temporal_hyperedge_emb = self.temporal_hyperedge_MP(cur,pre,temporal_hyperedge_incidence)
        node_emb = self.node_mp(cur,spatial_hyperedge_emb,temporal_hyperedge_emb)
        return node_emb,temporal_hyperedge_loss+spatial_hyperedge_loss



class Model(nn.Module):
    """
    multi-timestamp training
    """

    def __init__(self,win_size,h_dim = 256,n_cats = 5,recons_lambda = 0.1):
        super(Model, self).__init__()
        self.win_size = win_size
        self.time_cursor = TimeBlock()
        self.predictor = Predictor(h_dim,n_cats = n_cats)
        self.readout = Readout(h_dim)
        self.recons_lambda = recons_lambda

    def forward(self, node_fea):
        recon_loss = 0
        for i in range(self.win_size-1):
            if i == 0:
                pre_node = node_fea[0]
                cur_node = node_fea[1]
                cur_node_emb,r_loss = self.time_cursor(pre_node, cur_node)
                recon_loss += r_loss
            else:
                cur_node = node_fea[i + 1].contiguous()
                pre_node = cur_node_emb.contiguous()
                cur_node_emb,r_loss = self.time_cursor(pre_node, cur_node)
                recon_loss += r_loss
        graph_emb = self.readout(cur_node_emb,node_fea[-1])
        logits = self.predictor(graph_emb)
        return logits,recon_loss*self.recons_lambda




if __name__ == "__main__":
    pass



